Towards Inference Delivery Networks: Distributing Machine Learning with Optimality Guarantees

An increasing number of applications rely on complex inference tasks that are based on machine learning (ML). Currently, there are two options to run such tasks: either they are served directly by the end device (e.g., smartphones, IoT equipment, smart vehicles), or offloaded to a remote cloud. Both options may be unsatisfactory for many applications: local models may have inadequate accuracy, while the cloud may fail to meet delay constraints. In this paper, we present the novel idea of inference delivery networks (IDNs), networks of computing nodes that coordinate to satisfy ML inference requests achieving the best trade-off between latency and accuracy. IDNs bridge the dichotomy between device and cloud execution by integrating inference delivery at the various tiers of the infrastructure continuum (access, edge, regional data center, cloud). We propose a distributed dynamic policy for ML model allocation in an IDN by which each node dynamically updates its local set of inference models based on requests observed during the recent past plus limited information exchange with its neighboring nodes. Our policy offers strong performance guarantees in an adversarial setting and shows improvements over greedy heuristics with similar complexity in realistic scenarios.

==> sections/andrea-notes.tex <==

\todoi{aa: I am not sure this capacity model is realistic. $c^v$ is introduced as the ``number of GPUs'', while the model complexity is represented as $s_{m}^v$, since in the previous equation we do a comparison between $s_{m}^v$ and $c^v$, I assume that $s_{m}$ is a sort of ``number of GPUs'' needed for model $M_{i,q}$ to make inferences. Is my interpretation correct? (still, it is unclear in the description). However, if my interpretation is correct, this would mean that model $M_{i,q_1}$ would need a certain number $s_{i,q_1}$ of GPUs to run, while model $M_{i,q_2}$ would need a different number $s_{i,q_1}$ of GPUs to run. In this sense, we would reduce models in order for them to run with a smaller number of GPUs. \\
However, this is not the motivation why people reduce models~\cite{Hinton2015,Han2015a,Ravi2017,Ravi2018}. It is not like that for a complex model we need 10 GPUs, while for a small model 1 GPU is ok. Instead, for a complex model we need a big and expensive GPU, while for a small model we  are ok with just one small GPU. It is not the number of GPUs that matter, in my understanding, but the type of GPU, how big (and expensive) they are. Therefore, if you have a complex model, you will not be able to run it on 1000 small GPUs. You need one big GPU. This is not captured by the model (provided what I am saying is correct).\\
\textbf{Suggestion: maybe we can take this assignment restriction into account by keeping the model exactly as it is: we just impose in the input parameters that the service cost $a_{i,q}^v$ is $\infty$ if the node $v$ has a complexity that is too limited to host a model with that quality $q$. What would you think about this solution?}\\
gn: thanks Andrea. Now we talk generically of available GPU memory and maximum throughput in terms of instructions per seconds.\\
Each model has multiple dimensions, but we assume that there is a dominant constraint and that $s_{i,q}$ is the model dimension corresponding to this constraint. It is true that the dominant constraint could be different at each node. Question (mostly for Tareq and Gabriele): can the theory  handle node's dependent size? if we we could have $s_{i,q}^v$ to capture that the different nodes can have different constraints (for one can be the memory, for another the computation). Or perhaps in this section we could have in any case $s_{i,q}^v$ to present a general model and then we could say that theoretical results hold for  $s_{i,q}^v$ not a function of $v$.\\
Andrea, I would not introduce the separate assignment constraints in terms of $b_{i,q}^v$.\\
As far as I understand our problem is not a multiple knapsack problem with or without assignments (we do not want to distribute a set of objects across multiple knapsacks), but a problem
with multiple knapsack constraints.
}
